Structure-Grounded Pretraining for Text-to-SQL

Learning to capture text-table alignment is essential for tasks like text-to-SQL. A model needs to correctly recognize natural language references to columns and values and to ground them in the given database schema. In this paper, we present a novel weakly supervised Structure-Grounded pretraining framework (StruG) for text-to-SQL that can effectively learn to capture text-table alignment based on a parallel text-table corpus. We identify a set of novel prediction tasks: column grounding, value grounding and column-value mapping, and leverage them to pretrain a text-table encoder. Additionally, to evaluate different methods under more realistic text-table alignment settings, we create a new evaluation set Spider-Realistic based on Spider dev set with explicit mentions of column names removed, and adopt eight existing text-to-SQL datasets for cross-database evaluation. STRUG brings significant improvement over BERT-LARGE in all settings. Compared with existing pretraining methods such as GRAPPA, STRUG achieves similar performance on Spider, and outperforms all baselines on more realistic sets. The Spider-Realistic dataset is available at https://doi.org/10.5281/zenodo.5205322.

==> sections/introduction_old.tex <==
\section{Introduction}
The rapid development of large scale pretrained language models (PLMs) in recent years has benefited a wide range of NLP tasks, from simple sentence classification to complex sentence generation and question answering. Early study shows that directly incorporating PLMs trained on massive open domain text corpus with unsupervised objectives as feature extractor layer can already achieved superior performance across many tasks. More recently, great attention has been paid to better leverage these models and adopt them to target domains and tasks has drawn great attention.

Adaptation for tasks involving only plain text is relatively easy, as they can usually solved with a simple classifier on top of the LM and the data format is unchanged. Both domain-adaptive pretraining with the same unsupervised objectives on in-domain text corpus and multi-task learning with task specific objectives and cross-task data have shown promising results. On the contrary, fine-tuning for complex tasks that requires reasoning over both text and structured data is much more challenging. A typical example is text-to-SQL, where the model takes as input the user natural language query with the structured database schema, and translate it into a SQL query to be executed over the DB. The key challenge here is to learn the alignment between NL utturance and DB schema. However, this usually requires supervised data with SQL queries, which is expensive to annotate. Two recent works attempt to solve this problem by leveraging unsupervised sentence-table pairs scraped from the Web. They extend the BERT model with special designed encoder and pretraining objective to handle the additional structured DB schema input. However, they still rely on the random mask objective which cannot learn the alignment information efficiently and requires tremendous computing resource.

Inspired by the success of multi-task learning and design of existing text-to-SQL models, in this work, we propose to fine-tune PLMs with multiple tasks related to text-to-SQL using weakly supervised data. We identify three important subtasks of text-to-SQL: constraint value prediction, constraint column prediction and value column mapping. Constraint value prediction and constraint column prediction aim to identify the values in the NL utterance and columns in the DB schema that are used as constraints in SQL query (e.g., columns and values in WHERE clause), while value column mapping tries to capture the alignment between them. We leverage an existing parallel corpus that contains sentences and tables collected from Wikipedia and obtain labels for the subtasks via weak supervision to alleviate the problem of expensive annotation. We design heuristics for two scenarios: (1) We use the original sentence and table pairs scraped from Wikipedia and automatically annotate them with heuristics like sentence token and cell value matching. (2) We use the revised sentences that only contains
information related to the tables and cell annotations that have cells mentioned in the sentences highlighted. Such annotations are much easier to get compared with having experts writing SQL queries.

We start with the pretrained BERT model, and fine-tune it using the weakly supervised dataset for the three subtasks. Thanks to the weakly supervised objective, our approach is much more efficient compared with previous unsupervised methods, and generally converges well after only fine-tuning for five epochs. Since we do not make modifications to the language model architecture, the fine-tuned model can be easily plugged into existing text-to-SQL models.

Combined with state-of-the-art text-to-SQL model RAT-SQL, using our fine-tuned model as encoder significantly outperforms directly adopting pretrained BERT on the SPIDER dataset. To better demonstrate the superiority of our model, we also evaluate with multiple more challenging datasets that have much less explicit mention of constraint columns.

Our fine-tuning method can also help reduce the need for large amount of costly supervised training data. Experiment results on the WikiSQL benchmark show that using our fine-tuned model can boost the model performance by a large margin when only limited training data is available and brings consistent improvement over the baseline using the same amount of training data.

\textcolor{red}{To Discuss:\\
1. Motivation of the work
\begin{itemize}
    \item Task/domain adaptation of PLMs is popular \citep{liu2019multi,gururangan2020don}. Two recent works \citep{herzig2020tapas,yin2020tabert} study the problem for semantic parsing on tables via pretraining on parallel sentence-table corpus. However, the unsupervised pretraining objective they use is inefficient and is not designed to learn the alignment between sentences and tables. Motivated by this we design our pretraining method. We experiment under two settings: 1. To demonstrate that our pretraining can improve text-to-SQL performance, we experiment with spider +  several more challenging datasets. 2. Two show that our method can reduce the need for labeled data, we experiment on WikiSQL with sampled subset.
    \item One of the key challenges of text-to-SQL is to learn the alignment between texts and DB schemas, and select the correct value and columns to use in the generated query. Given this observation, we aim to leverage an existing sentence-table parallel corpus to learn such alignment by pretraining with three subtasks. Also we notice that existing text-to-SQL benchmark like spider simplify the problem by explicitly mention the values and columns in the question. To better demonstrate the advantage of using our pretraining, we create a more challenging evaluation set based on original spider dev set and also include some other DBs used in \cite{suhr2020exploring}. In addition, experiments on WikiSQL show that such alignment knowledge learned in pretraining can reduce the need for large amount of labeled training data.
\end{itemize}
2. If we make the main contribution of this paper as new pretraining technique for text-to-SQL, should we compare with TaBERT (replace the encoder in ratsql with TaBERT). TAPAS is not suitable for complex sql query generation since it only has one cell selection and one aggregation operation.\\
3. Should we highlight the new evaluation set and use of other DBs in introduction.\\
4. How to explain our handling of columns in select clause, as we do not consider them when creating the new evaluation set. Intuitively, our pretraining won't help much for columns in select, and the experiment results also verify this. Should we mention and explain this in the introduction.
}

